Controllable Text Generation for Large Language Models: A Survey

In Natural Language Processing (NLP), Large Language Models (LLMs) have demonstrated high text generation quality. However, in real-world applications, LLMs must meet increasingly complex requirements. Beyond avoiding misleading or inappropriate content, LLMs are also expected to cater to specific user needs, such as imitating particular writing styles or generating text with poetic richness. These varied demands have driven the development of Controllable Text Generation (CTG) techniques, which ensure that outputs adhere to predefined control conditions--such as safety, sentiment, thematic consistency, and linguistic style--while maintaining high standards of helpfulness, fluency, and diversity. This paper systematically reviews the latest advancements in CTG for LLMs, offering a comprehensive definition of its core concepts and clarifying the requirements for control conditions and text quality. We categorize CTG tasks into two primary types: content control and attribute control. The key methods are discussed, including model retraining, fine-tuning, reinforcement learning, prompt engineering, latent space manipulation, and decoding-time intervention. We analyze each method's characteristics, advantages, and limitations, providing nuanced insights for achieving generation control. Additionally, we review CTG evaluation methods, summarize its applications across domains, and address key challenges in current research, including reduced fluency and practicality. We also propose several appeals, such as placing greater emphasis on real-world applications in future research. This paper aims to offer valuable guidance to researchers and developers in the field. Our reference list and Chinese version are open-sourced at https://github.com/IAAR-Shanghai/CTGSurvey.

==> figures/forest.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{forest}
for tree={
    grow=east,
    parent anchor=east,
    child anchor=west,
    draw,
    rounded corners,
    align=center,
    l sep+=10pt,
    s sep+=5pt,
    font=\sffamily,
    inner xsep=10pt,
    inner ysep=4pt,
    fill=blue!10,
    draw=blue!50,
    line width=1pt,
    edge path={
        \noexpand\path [draw=blue!50, thick, -] (!u.south east) |- (.child anchor)\forestoption{edge label};
    }
}
[Agent Architecture
    [Memory
        [Memory Sources
            [User-Agent Interaction
                [\textit{e.g. Xu et al. (2022), Jiang et al., RoleInteract (Chen et al., 2024a)}]
            ]
            [Agent-Agent Interaction
                [\textit{e.g. Maas et al. (2023), Generative Agent (Park et al., 2023)}]
            ]
        ]
        [Memory Usage
            [Retrieval-based
                [\textit{e.g. PLATO-LTM (Xu et al., 2022), Bae et al. (2022)}]
            ]
            [Compressive-based
                [\textit{e.g. COMEDY (Chen et al., 2024b), Wang et al. (2023d)}]
            ]
        ]
    ]
    [Planning
        [Planning Formulation
            [\textit{e.g. Dasgupta et al. (2023), Wang et al. (2023d), Inner Monologue (Huang et al., 2022a)}]
        ]
        [Planning Reflection
            [\textit{e.g. Generative Agent (Park et al., 2023), MORTISE (Tang et al., 2024), Wu et al. (2022)}]
        ]
    ]
    [Action
        [\textit{e.g. RoleLLM (Wang et al., 2023e), Humanoid Agents (Wang et al., 2023g), Shen et al. (2024a)}]
    ]
]
\end{forest}
}
\caption{The main content flow and categorization of Agent Architecture.}
\label{fig:agent-architecture}
\end{figure*}
